F-FOMAML: GNN-Enhanced Meta-Learning for Peak Period Demand Forecasting with Proxy Data

Demand prediction is a crucial task for e-commerce and physical retail businesses, especially during high-stake sales events. However, the limited availability of historical data from these peak periods poses a significant challenge for traditional forecasting methods. In this paper, we propose a novel approach that leverages strategically chosen proxy data reflective of potential sales patterns from similar entities during non-peak periods, enriched by features learned from a graph neural networks (GNNs)-based forecasting model, to predict demand during peak events. We formulate the demand prediction as a meta-learning problem and develop the Feature-based First-Order Model-Agnostic Meta-Learning (F-FOMAML) algorithm that leverages proxy data from non-peak periods and GNN-generated relational metadata to learn feature-specific layer parameters, thereby adapting to demand forecasts for peak events. Theoretically, we show that by considering domain similarities through task-specific metadata, our model achieves improved generalization, where the excess risk decreases as the number of training tasks increases. Empirical evaluations on large-scale industrial datasets demonstrate the superiority of our approach. Compared to existing state-of-the-art models, our method demonstrates a notable improvement in demand prediction accuracy, reducing the Mean Absolute Error by 26.24% on an internal vending machine dataset and by 1.04% on the publicly accessible JD.com dataset.

==> MAML_defs.tex <==
%% editing comment
\newcommand{\cmt}[1]{{\footnotesize\textcolor{red}{#1}}}
\newcommand{\note}[1]{\cmt{Note: #1}}
\newcommand{\todo}[1]{\cmt{TO-DO: #1}}
\newcommand{\sergey}[1]{\cmt{Sergey: #1}}
\newcommand{\chelsea}[1]{\cmt{Chelsea: #1}}
\newcommand{\pieter}[1]{\cmt{Pieter: #1}}
\newcommand{\review}[1]{\noindent\textcolor{red}{$\rightarrow$ #1}}
\newcommand{\response}[1]{\noindent{#1}}

%% ignore text
\long\def\ignorethis#1{}

%% abbreviations
% \newcommand{\etal}{{et~al.}\ }
% \newcommand{\eg}{e.g.\ }
% \newcommand{\ie}{i.e.\ }
% \newcommand{\nth}{\text{th}}
\newcommand{\pr}{^\prime}
\newcommand{\tr}{^\mathrm{T}}
\newcommand{\inv}{^{-1}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\gauss}{\mathcal{N}}
\newcommand{\norm}[1]{\left|#1\right|}
\newcommand{\trace}{\text{tr}}

%% reference shortcuts
\newcommand{\figtodo}[1]{\framebox[0.8\columnwidth]{\rule{0pt}{1in}#1}}
% \newcommand{\figref}[1]{Figure~\ref{fig:#1}}
%\renewcommand{\eqref}[1]{Equation~(\ref{eq:#1})}
% \newcommand{\secref}[1]{Section~\ref{sec:#1}}

%% section definitions.
\newcommand{\secpaperlin}{5.1}
\newcommand{\eqnpapergradmul}{3}
\newcommand{\eqnpapergrads}{4}
\newcommand{\applinhess}{A}
\newcommand{\applqr}{B}
\newcommand{\appfastgrad}{C}

%% general math definitions
\newcommand{\vnorm}[1]{\|#1\|}
\newcommand{\lscnorm}[1]{\ell_{12}(#1)}
\newcommand{\costnorm}{r_\ell}

%% BADMM penalties
\newcommand{\badmmtraj}{\phi^{\trajdist}}
\newcommand{\badmmpol}{\phi^{\params}}
\newcommand{\lagtraj}{\mathcal{L}_{\trajdist}}
\newcommand{\lagpol}{\mathcal{L}_{\params}}

\newcommand{\energy}{\mathcal{E}}

%% shortcuts for paper
\newcommand{\admmrate}{\alpha}
\newcommand{\cluster}{c}
\newcommand{\dualstep}{\eta}
\newcommand{\polwt}{\lambda}
\newcommand{\lgmult}{\lambda}
\newcommand{\lgmultt}{\lambda_t}
\newcommand{\lgmu}{\lambda_\mu}
\newcommand{\lgmut}{\lambda_{\mu t}}
\newcommand{\admmrho}{\nu}
\newcommand{\lagrangian}{\mathcal{L}_{\text{traj}}}
\newcommand{\lagrangiangps}{\mathcal{L}_{\text{GPS}}}
\newcommand{\trajdist}{p}
\newcommand{\policy}{\pi}
\newcommand{\policytraj}{\pi_{\traj}}
\newcommand{\return}{J}
\newcommand{\params}{\theta}
\newcommand{\reward}{R}
\newcommand{\cost}{\ell}
\newcommand{\state}{\mathbf{x}}
\newcommand{\action}{\mathbf{a}}
\newcommand{\obs}{\mathbf{o}}
\newcommand{\opt}{\mathcal{R}}
\newcommand{\hstate}{\hat{\mathbf{x}}}
\newcommand{\haction}{\hat{\mathbf{u}}}
\newcommand{\states}{\mathcal{X}}
\newcommand{\actions}{\mathcal{A}}
%\renewcommand{\path}{\zeta}
\newcommand{\traj}{\tau}
\newcommand{\covar}{\Sigma}
\newcommand{\trajmu}{\mu^\trajdist}
\newcommand{\trajmut}{\mu^\trajdist_t}
\newcommand{\polmu}{\mu^\policy}
\newcommand{\polsig}{\Sigma^\policy}
\newcommand{\polmut}{\mu^\policy_t}
\newcommand{\polmudiffavgt}{\hat{\mu}^\policy_t}
\newcommand{\polsigt}{\Sigma^\policy_t}
\newcommand{\polgrad}{\polmu_\state}
\newcommand{\polgradt}{\polmu_{\state t}}
\newcommand{\polgradavgt}{\hat{\mu}^\policy_{\state t}}
\newcommand{\ucovar}{\mathbf{C}}
\newcommand{\xcovar}{\mathbf{S}}
\newcommand{\ucovart}{\mathbf{C}_t}
\newcommand{\xcovart}{\mathbf{S}_t}
\newcommand{\hxcovart}{\hat{\mathbf{S}}_t}
\newcommand{\xcovartp}{\mathbf{S}_{t+1}}
\newcommand{\xucovar}{\Sigma}
\newcommand{\xucovart}{\Sigma_t}
\newcommand{\xcovarchol}{\mathbf{L}}
\newcommand{\xcovarcholt}{\xcovarchol_t}
\newcommand{\samp}{\mathbf{s}}
\newcommand{\sampti}{\samp_{ti}}
\newcommand{\sampdist}{q}
\newcommand{\obj}{\mathcal{L}}
\newcommand{\objut}{\obj_{\action t}}
\newcommand{\objuut}{\obj_{\action,\action t}}
\newcommand{\objxt}{\obj_{\state t}}
\newcommand{\objxxt}{\obj_{\state,\state t}}
\newcommand{\objucovart}{\obj_{\ucovar t}}
\newcommand{\objxcovart}{\obj_{\xcovar t}}
\newcommand{\objxcovartp}{\obj_{\xcovar t+1}}
\newcommand{\feedback}{\mathbf{K}}
%\newcommand{\example}{\text{ex}}
\newcommand{\detpolicy}{g}
\newcommand{\wtreg}{w_r}
\newcommand{\velx}{v_x}
\newcommand{\posy}{p_y}
\newcommand{\pos}{\mathbf{p}}
\newcommand{\torquepen}{w_\action}
\newcommand{\pospen}{w_\pos}
\newcommand{\velpen}{w_v}
\newcommand{\heightpen}{w_h}
\newcommand{\all}{{1..T}}

\newcommand{\channel}{c}
\newcommand{\softmax}{\mathbf{s}}
\newcommand{\softmaxpix}{s_{cij}}
\newcommand{\responsemap}{\mathbf{a}}
\newcommand{\responsepix}{a_{cij}}
\newcommand{\responsepixprime}{a_{ci'j'}}

\newcommand{\innerterm}{\xi}

\newcommand{\second}{\text{s}}
\newcommand{\ms}{\text{m/s}}
\newcommand{\meter}{\text{m}}

\newcommand{\kl}{D_\text{KL}}
\newcommand{\tv}{D_\text{TV}}
\newcommand{\ent}{\mathcal{H}}
\newcommand{\rdist}{\rho}

\newcommand{\fc}{f_c}
\newcommand{\fx}{f_\state}
\newcommand{\fu}{f_\action}
\newcommand{\fct}{f_{c t}}
\newcommand{\fxt}{f_{\state t}}
\newcommand{\fut}{f_{\action t}}
\newcommand{\fy}{f_{\state\action}}
\newcommand{\fyt}{f_{\state\action t}}
\newcommand{\rx}{\reward_\state}
\newcommand{\ru}{\reward_\action}
\newcommand{\rxx}{\reward_{\state,\state}}
\newcommand{\ruu}{\reward_{\action,\action}}
\newcommand{\rux}{\reward_{\action,\state}}
\newcommand{\rxt}{\reward_{\state t}}
\newcommand{\rut}{\reward_{\action t}}
\newcommand{\rxxt}{\reward_{\state,\state t}}
\newcommand{\ruut}{\reward_{\action,\action t}}
\newcommand{\ruxt}{\reward_{\action,\state t}}
\newcommand{\Qx}{Q_\state}
\newcommand{\Qu}{Q_\action}
\newcommand{\Qy}{Q_{\state\action}}
\newcommand{\Qxx}{Q_{\state,\state}}
\newcommand{\Quu}{Q_{\action,\action}}
\newcommand{\Qux}{Q_{\action,\state}}
\newcommand{\Qxu}{Q_{\state,\action}}
\newcommand{\Qyy}{Q_{\state\action,\state\action}}
\newcommand{\Qxt}{Q_{\state t}}
\newcommand{\Qut}{Q_{\action t}}
\newcommand{\Qyt}{Q_{\state\action t}}
\newcommand{\Qxxt}{Q_{\state,\state t}}
\newcommand{\Quut}{Q_{\action,\action t}}
\newcommand{\Quxt}{Q_{\action,\state t}}
\newcommand{\Qxut}{Q_{\state,\action t}}
\newcommand{\Qyyt}{Q_{\state\action,\state\action t}}
\newcommand{\Vx}{V_\state}
\newcommand{\Vxx}{V_{\state,\state}}
\newcommand{\Vxt}{V_{\state t}}
\newcommand{\Vxxt}{V_{\state,\state t}}
\newcommand{\Vxtp}{V_{\state t+1}}
\newcommand{\Vxxtp}{V_{\state,\state t+1}}
\newcommand{\kpol}{\mathbf{k}}
\newcommand{\Kpol}{\mathbf{K}}
\newcommand{\passivedyn}{p}
\newcommand{\lmdp}{\mathcal{G}}
\newcommand{\samples}{\mathcal{S}}
\newcommand{\ft}{f_t}
\newcommand{\noise}{\mathbf{F}}
\newcommand{\siglinmatt}{\mathbf{M}}


\newcommand{\objKt}{\obj_{\Kpol t}}
\newcommand{\objKht}{\obj_{\hat{\Kpol} t}}
\newcommand{\polsampcovar}{\mathbf{C}_t}
\newcommand{\cholin}{\mathbf{D}_t}

\newcommand{\costgrad}{\cost_{\state\action}}
\newcommand{\costhess}{\cost_{\state\action,\state\action}}
\newcommand{\tcostgrad}{\tilde{\cost}_{\state\action}}
\newcommand{\tcosthess}{\tilde{\cost}_{\state\action,\state\action}}
\newcommand{\costxx}{\cost_{\state,\state}}
\newcommand{\costuu}{\cost_{\action,\action}}
\newcommand{\costxu}{\cost_{\state,\action}}
\newcommand{\costux}{\cost_{\action,\state}}
\newcommand{\costxxt}{\cost_{\state,\state t}}
\newcommand{\costuut}{\cost_{\action,\action t}}
\newcommand{\costxut}{\cost_{\state,\action t}}
\newcommand{\costuxt}{\cost_{\action,\state t}}
\newcommand{\costxt}{\cost_{\state t}}
\newcommand{\costut}{\cost_{\action t}}
\newcommand{\costgradu}{\cost_\action}
\newcommand{\costhessu}{\cost_{\action,\action}}

\newcommand{\costgradt}{\cost_{\state\action t}}
\newcommand{\costhesst}{\cost_{\state\action,\state\action t}}
\newcommand{\tcostgradt}{\tilde{\cost}_{\state\action t}}
\newcommand{\tcosthesst}{\tilde{\cost}_{\state\action,\state\action t}}
\newcommand{\costgradut}{\cost_{\action t}}
\newcommand{\costhessut}{\cost_{\action,\action t}}

\newcommand{\tcgradt}{\tilde{c}_{\state\action t}}
\newcommand{\tchesst}{\tilde{c}_{\state\action,\state\action t}}

\newcommand{\choldiff}{\text{choldiff}}

% quick shortcut definitions.
\newcommand{\st}{\state_t}
\newcommand{\at}{\action_t}
\newcommand{\ot}{\obs_t}
\newcommand{\sti}{\state_{ti}}
\newcommand{\ati}{\action_{ti}}
\newcommand{\sth}{\hstate_t}
\newcommand{\ath}{\haction_t}

% line search stuff
\newcommand{\points}{\mathbf{p}}
\newcommand{\Cost}{\langle\ell\rangle}
\newcommand{\Penalty}{a}
\newcommand{\Rate}{b}

% Prior stuff.
\newcommand{\empsig}{\hat{\Sigma}}
\newcommand{\empmu}{\hat{\mu}}
\newcommand{\empn}{N}
\newcommand{\priorphi}{\mathbf{\Phi}}
\newcommand{\priormu}{\mu_0}
\newcommand{\priormut}{\mu_{0t}}
\newcommand{\priorm}{m}
\newcommand{\priorn}{n_0}
\newcommand{\datapt}{\mathbf{p}}
\newcommand{\ddpdiscount}{\gamma}
\newcommand{\onlinediscount}{\beta}
\newcommand{\xxt}{\Delta}
\newcommand{\net}{\bar{f}}
\newcommand{\sigt}{\bar{\Sigma}_{\state\action,\state\action}}
\newcommand{\sigp}{\bar{\Sigma}_{\state\pr,\state\pr}}

